Leveraging Joint Spectral and Spatial Learning with MAMBA for Multichannel Speech Enhancement

In multichannel speech enhancement, effectively capturing spatial and spectral information across different microphones is crucial for noise reduction. Traditional methods, such as CNN or LSTM, attempt to model the temporal dynamics of full-band and sub-band spectral and spatial features. However, these approaches face limitations in fully modeling complex temporal dependencies, especially in dynamic acoustic environments. To overcome these challenges, we modify the current advanced model McNet by introducing an improved version of Mamba, a state-space model, and further propose MCMamba. MCMamba has been completely reengineered to integrate full-band and narrow-band spatial information with sub-band and full-band spectral features, providing a more comprehensive approach to modeling spatial and spectral information. Our experimental results demonstrate that MCMamba significantly improves the modeling of spatial and spectral features in multichannel speech enhancement, outperforming McNet and achieving state-of-the-art performance on the CHiME-3 dataset. Additionally, we find that Mamba performs exceptionally well in modeling spectral information.

==> Sections/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}

Multichannel speech enhancement (SE) is a critical and challenging research topic in speech signal processing. 
% With the rapid advancement of communication technologies and artificial intelligence, improving speech quality and intelligibility has become increasingly important across various applications, such as teleconferencing systems, automatic speech recognition, and hearing aids. 
% However, in real-world environments, speech signals are often corrupted by background noise and reverberation, which significantly degrade the clarity and intelligibility of speech.
In addition to the spectral information from each channel, the spatial information captured by multiple microphone arrays is an important cue for multichannel speech enhancement. 
Compared to single channel methods\cite{wang2018supervisedspeechseparationbased, choi2019phaseawarespeechenhancementdeep, Hao_2021, hu2020dccrndeepcomplexconvolution, lu13_interspeech}, multichannel techniques have the potential to significantly enhance speech quality by effectively incorporating both spatial and spectral information.

% In recent years, significant progress has been made in multichannel speech enhancement. 
% Traditional methods, such as beamforming\cite{bf4cc37f50814371a3bcb2b5f44d08ec} and multichannel Wiener filtering\cite{1542105}, have laid a solid foundation for advancements in the field. 
% Beamforming operates on the principle of spatial filtering, leveraging time and phase differences in the signals captured by the microphone array to enhance speech from a specific direction. 
% Multichannel Wiener filtering is often combined with spatial features, such as beamformed signals, to suppress noise in the frequency domain further.
% With the rise of deep learning, numerous neural network-based approaches have emerged. 
% One promising direction is neural beamforming\cite{erdogan16_interspeech,7471664}, which integrates deep learning with traditional multichannel beamforming techniques. 
% In this approach, neural networks generate time- and frequency-domain masks to separate speech and noise. These masks are then used to apply beamformers that linearly combine the multichannel inputs, ultimately predicting clean speech.
% Some techniques\cite{7886357,8540037} allow for the direct incorporation of inter-channel time/phase/level(ITD/IPD/ILD) differences into single-channel speech enhancement networks, enabling more effective utilization of spatial information. 

% In recent years, significant progress has been made in multichannel speech enhancement.
Traditional multichannel SE includes beamforming \cite{bf4cc37f50814371a3bcb2b5f44d08ec,erdogan16_interspeech,7471664} and multichannel Wiener filtering\cite{1542105}.
Some techniques \cite{7886357,8540037} allow for the direct incorporation of inter-channel time/phase/level(ITD/IPD/ILD) differences into single-channel speech enhancement networks, enabling more effective utilization of spatial information. 
Spatial and spectral information across multiple channels are important for multi-channel speech enhancement.
Spatial information refers to the differences in the sound signal captured by multiple microphones, which helps determine the location of sound sources. 
This allows systems to distinguish between speech and noise based on direction. 
Spectral information, on the other hand, refers to the frequency content of the signal, helping separate speech from noise by analyzing different frequency bands. 
Combining both spatial and spectral data improves the accuracy of speech enhancement.
Recently, there are neural networks specifically designed to process spatial and spectral information across multiple channels. 
Notably, this advancement is exemplified by mechanisms such as the channel attention approach introduced by Bahareh Tolooshams \cite{tolooshams2020channelattentiondenseunetmultichannel}.
In addition, specific neural networks are designed to specifically target the spatial distinctions between narrowband speech and noise\cite{li2020narrowbanddeepfilteringmultichannel,8937218}, further optimizing spatial information processing. 
The spectral domain is another crucial feature for differentiating clean speech from noise. 
Researchers have demonstrated that both full-band and sub-band regions contain valuable spectral information\cite{xiong22_interspeech}. 
The state-of-the-art performance is achieved by modeling the spatial information in narrow-band and full-band frequencies while effectively combining sub-band and full-band features\cite{yang2022mcnetfusemultiplecues}.

A recent state-space model incorporating a selection mechanism known as Mamba\cite{gu2024mambalineartimesequencemodeling} has demonstrated state-of-the-art performance in single-channel speech enhancement\cite{li2024spmambastatespacemodelneed,chao2024investigationincorporatingmambaspeech}. 
Building on this, SpatialNet introduces a variant of Mamba tailored for long-term streaming multichannel speech enhancement\cite{quan2024multichannellongtermstreamingneural}, particularly suited for scenarios involving stationary and moving speakers. 
However, SpatialNet focuses primarily on utilizing spatial information. 
Research exploring the joint use of equally important spatial and spectral features in state-space models for multichannel speech enhancement remains unexplored.

This study proposes a novel multi-channel speech enhancement system based on Mamba, which aims to effectively capture spatial and spectral information. 
We develop causal and non-causal versions of the system to meet practical application requirements. 
The specially designed Mamba module is dedicated to modeling spatial and spectral characteristics. 
Extensive experimental results show that on the CHiME-3 dataset, our method outperforms the state-of-the-art network MCNet in terms of all speech enhancement metrics.





==> tables/figure1.tex <==
% \begin{figure*}[ht]
%     \centering
%     \begin{minipage}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/window_type.png} % Replace with your image file name
%         % \caption{Different models.}
%         \label{fig:image1}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/model_type.png} % Replace with your image file name
%         % \caption{Different windows.}
%         \label{fig:image2}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/model_type_mac.png} % Replace with your image file name
%         % \caption{Different windows.}
%         \label{fig:image3}
%     \end{minipage}
%     % \vspace{-8pt}
%     \caption{From the left to right, figures denote OVL scores for various window types and models, and MACs/sec for models.}
%     % \vspace{-8pt}
%     \label{fig:all}
% \end{figure*}


\begin{figure}[tb]
    \centering
    \begin{minipage}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,clip,trim=0 5 0 4]{figures/results_all.png}
        \label{fig:image1}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth,clip,trim=0 5 0 4]{figures/results_macs.png}
        \label{fig:image2}
    \end{minipage}
    \caption{Overall results for various low latency methods and model sizes (left), and MACs/sec for models (right).}
    % \vspace{-8pt}
    \label{fig:all}
\end{figure}

==> tables/future_predict.tex <==
\begin{table}[ht]
\centering
\caption{Analysis for predicting future frames. All models use the input window size of 20ms.}
% \vspace{2pt}
\label{tab:predict}
\adjustbox{width=0.5\textwidth}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model name} & \textbf{oWin (ms)} & \textbf{Target} & \textbf{SIG} & \textbf{BAK} & \textbf{OVR} \\
\midrule
asym-mask     & 3 & filtering  & 3.15 & 3.78 & 2.77 \\
asym-map      & 3 & mapping  & 3.10 & 3.74 & 2.70 \\
asym-map-pred & 6 & mapping  & 3.06 & 3.71 & 2.65 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/model_size.tex <==
\begin{table}[ht]
\centering
\caption{Comparison for different model sizes. The model architecture is CRUSE.}
% \vspace{2pt}
\label{tab:model_size}
\adjustbox{max width=\textwidth}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Model Name} & \textbf{iWin} & \textbf{oWin} & \textbf{SIG} & \textbf{BAK} & \textbf{OVR} \\
\midrule
sym-20ms & 20 & 20 & 3.18 & 3.78 & 2.79 \\
\midrule
sym-10ms & 10 & 10 & 3.16 & 3.81 & 2.79 \\
sym-5ms  & 5  & 5  & 3.12 & 3.77 & 2.74 \\
sym-3ms  & 3  & 3  & 3.12 & 3.77 & 2.74 \\
\midrule
asym-10ms & 20 & 10 & 3.15 & 3.78 & 2.77 \\
asym-5ms  & 20 & 5  & 3.13 & 3.77 & 2.75 \\
asym-3ms  & 20 & 3  & 3.15 & 3.78 & 2.77 \\
\midrule
asym-10ms-medium & 20 & 10 & 3.19 & 3.77 & 2.80 \\
asym-5ms-medium  & 20 & 5  & 3.16 & 3.80 & 2.78 \\
asym-3ms-medium  & 20 & 3  & 3.18 & 3.78 & 2.80 \\
\midrule
asym-10ms-large & 20 & 10 & 3.22 & 3.80 & 2.84 \\
asym-5ms-large  & 20 & 5  & 3.22 & 3.77 & 2.83 \\
asym-3ms-large  & 20 & 3  & 3.20 & 3.76 & 2.80 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/unet.tex <==
\begin{table}[tb]
\centering
\caption{Comparison between asymmetric and symmetric windows. The model architecture is UNet.}
% \vspace{2pt}
\label{tab:unet}
\adjustbox{width=0.3\textwidth}{
\begin{tabular}{cccccc}
\toprule
\textbf{iWin (ms)} & \textbf{oWin (ms)} & \textbf{SIG} & \textbf{BAK} & \textbf{OVR} \\
\midrule
20 & 20 & 2.80 & 3.74 & 2.47 \\
\midrule
10 & 10 & 2.71 & 3.61 & 2.35 \\
20 & 10 & 2.72 & 3.64 & 2.38 \\
\midrule
5  & 5  & 2.59 & 3.54 & 2.24 \\
20 & 5  & 2.66 & 3.57 & 2.30 \\
\midrule
3  & 3  & 2.49 & 3.53 & 2.16 \\
20 & 3  & 2.62 & 3.52 & 2.25 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/windows.tex <==

\renewcommand{\arraystretch}{0.8}
\begin{table*}[ht]
\centering
\caption{Comparison for different windows and models. iWin and oWin denote the input and output window lengths.}
\vspace{-8pt}
\label{tab:all}
\adjustbox{max width=0.95\textwidth}{
\begin{tabular}{cc|ccc|cc|ccc|ccccccc}
\toprule
\multirow{2}{*}{\textbf{Row}} & \multirow{2}{*}{\textbf{Model Name}} & \multirow{2}{*}{\textbf{iWin}} & \multirow{2}{*}{\textbf{oWin}} & \multirow{2}{*}{\textbf{Latency}} & \multirow{2}{*}{\textbf{Model Size}} & \multirow{2}{*}{\textbf{MACs}} & \multicolumn{3}{c}{\textbf{DNS blind set}} & \multicolumn{6}{c}{\textbf{simulated data}} \\
\cmidrule(lr){8-10} \cmidrule(lr){11-16}
 &  & & & & & & \textbf{SIG} & \textbf{BAK} & \textbf{OVR} & \textbf{SIG} & \textbf{BAK} & \textbf{OVR} & \textbf{PESQ} & \textbf{STOI (\%)} & \textbf{SISDR} \\
\midrule
A1 & sym-20ms & 20 & 20 & 20 & 0.625M & 230.27M & 3.18 & 3.78 & 2.79 & 2.87 & 4.03 & 2.46 & 2.22 & 84.45 & 10.52 \\
A2 & sym-10ms & 10 & 10 & 10 & 0.625M & 460.53M & 3.16 & 3.81 & 2.79 & 2.83 & 4.03 & 2.43 & 2.24 & 84.59 & 10.32 \\
A3 & sym-5ms & 5 & 5 & 5 & 0.625M & 921.06M & 3.12 & 3.77 & 2.74 & 2.78 & 4.02 & 2.38 & 2.21 & 84.46 & 9.94 \\
A4 & sym-3ms & 3 & 3 & 3 & 0.625M & 1.54G & 3.12 & 3.77 & 2.74 & 2.76 & 4.02 & 2.36 & 2.18 & 84.23 & 9.65 \\
\midrule
B1 & asym-10ms & 20 & 10 & 10 & 0.625M & 460.53M & 3.15 & 3.78 & 2.77 & 2.84 & 4.03 & 2.44 & 2.22 & 84.34 & 10.18 \\
B2 & asym-5ms & 20 & 5 & 5 & 0.625M & 921.06M & 3.13 & 3.77 & 2.75 & 2.81 & 4.03 & 2.41 & 2.16 & 84.20 & 10.06 \\
B3 & asym-3ms & 20 & 3 & 3 & 0.625M & 1.54G & 3.15 & 3.78 & 2.77 & 2.80 & 4.02 & 2.40 & 2.16 & 84.17 & 9.85 \\
\midrule
C1 & Learn-asym-10ms & 20 & 10 & 10 & 0.625M & 460.53M & 3.23 & 3.78 & 2.83 & 2.88 & 4.03 & 2.47 & 2.31 & 84.88 & 10.84 \\
C2 & Learn-asym-5ms & 20 & 5 & 5 & 0.625M & 921.06M & 3.19 & 3.81 & 2.82 & 2.80 & 4.03 & 2.40 & 2.31 & 85.02 & 10.64 \\
C3 & Learn-asym-3ms & 20 & 3 & 3 & 0.642M & 1.54G & 3.14 & 3.78 & 2.76 & 2.76 & 4.02 & 2.37 & 2.22 & 84.22 & 10.13 \\
\midrule
D1 & asym-same\_compute-10ms & 20 & 10 & 10 & 0.551M & 249.8M & 3.13 & 3.80 & 2.76 & 2.82 & 4.02 & 2.41 & 2.18 & 84.08 & 9.90 \\
D2 & asym-same\_compute-5ms & 20 & 5 & 5 & 0.157M & 235.04M & 3.08 & 3.71 & 2.68 & 2.76 & 4.01 & 2.36 & 2.10 & 83.04 & 9.29 \\
D3 & asym-same\_compute-3ms & 20 & 3 & 3 & 0.142M & 230.33M & 3.09 & 3.66 & 2.67 & 2.74 & 3.99 & 2.33 & 2.05 & 82.77 & 9.03 \\
\midrule
E1 & Mamba-20ms & 20 & 20 & 20 & 0.642M & - & 3.19 & 3.80 & 2.81 & 2.87 & 4.03 & 2.46 & 2.27 & 84.59 & 10.61 \\
E2 & Mamba-10ms & 10 & 10 & 10 & 0.642M & - & 3.10 & 3.77 & 2.72 & 2.81 & 4.02 & 2.40 & 2.21 & 83.96 & 10.16 \\
E3 & Mamba-5ms & 5 & 5 & 5 & 0.642M & - & 3.03 & 3.67 & 2.63 & 2.73 & 4.00 & 2.33 & 2.15 & 83.42 & 9.71 \\
\midrule
F1 & asym-10ms-medium & 20 & 10 & 10 & 2.32M & 1.09G & 3.19 & 3.77 & 2.80 & 2.85 & 4.02 & 2.44 & 2.30 & 84.75 & 10.56 \\
F2 & asym-5ms-medium & 20 & 5 & 5 & 2.32M & 2.20G & 3.16 & 3.80 & 2.78 & 2.84 & 4.03 & 2.43 & 2.19 & 84.15 & 10.07 \\
F3 & asym-3ms-medium & 20 & 3 & 3 & 2.32M & 3.66G & 3.18 & 3.78 & 2.80 & 2.82 & 4.02 & 2.42 & 2.22 & 84.68 & 10.16 \\
F4 & asym-10ms-large & 20 & 10 & 10  & 8.67M  & 3.28G & 3.22 & 3.80 & 2.84 & 2.87 & 4.04 & 2.47 & 2.33 & 85.24 & 10.70 \\
F5 & asym-5ms-large & 20 & 5 & 5 & 8.67M & 6.57G & 3.22 & 3.77 & 2.83 & 2.85 & 4.03 & 2.45 & 2.29 & 85.08 & 10.55 \\
F6 & asym-3ms-large & 20 & 3 & 3 & 8.67M & 10.95G & 3.20 & 3.76 & 2.80 & 2.82 & 4.01 & 2.42 & 2.27 & 84.89 & 10.34 \\
\midrule
G1 & asym-3ms-mapping &	20 &3 &3 & 0.625M &	1.54G &	3.10 &	3.74 &	2.70 &	2.70 &	4.01 &	2.28 &	1.91 &	81.85 &	8.19 \\
G2 & asym-6ms-predict &	6 &	6 &	3	& 0.625M &	767.57M &	3.06 &	3.71 &	2.65 & 2.71 &	4.01 &	2.29 &	2.09 &	83.35 &	9.34 \\
\midrule
H1 & FBE-10ms &	- &	- &	10	& 0.656M &	256.1M &	3.15 &	3.68 &	2.72 & 2.80 &	3.93 &	2.36 &	2.05 &	82.98 &	8.91 \\
H2 & FBE-5ms &	- &	- &	5	& 0.644M &	590.6M &	3.11 &	3.65 &	2.68 & 2.75 & 3.93 & 2.32 & 2.00 &	82.90 &	8.60 \\
H3 & FBE-2.5ms &	- &	- &	2.5	& 0.637M &	1.098G &	3.07 &	3.58 &	2.62 & 2.71 & 3.89 &	2.27 & 1.89 & 81.73 & 7.80 \\
\bottomrule
\end{tabular}
}
\end{table*}

